FOAL: Fine-grained Contrastive Learning for Cross-domain Aspect Sentiment Triplet Extraction

Aspect Sentiment Triplet Extraction (ASTE) has achieved promising results while relying on sufficient annotation data in a specific domain. However, it is infeasible to annotate data for each individual domain. We propose to explore ASTE in the cross-domain setting, which transfers knowledge from a resource-rich source domain to a resource-poor target domain, thereby alleviating the reliance on labeled data in the target domain. To effectively transfer the knowledge across domains and extract the sentiment triplets accurately, we propose a method named Fine-grained cOntrAstive Learning (FOAL) to reduce the domain discrepancy and preserve the discriminability of each category. Experiments on six transfer pairs show that FOAL achieves 6% performance gains and reduces the domain discrepancy significantly compared with strong baselines. Our code will be publicly available once accepted.

==> chapters/0_abstract.tex <==
\begin{abstract}
Aspect Sentiment Triplet Extraction (ASTE) aims to identify sentiment triplets from a given review. Prior works on ASTE typically rely on a large amount of labeled data, which is impractical for applications. Therefore, we investigate ASTE in the cross-domain setting, which adapts existing models trained on a resource-rich source domain to a resource-poor target domain. 
The key challenge for cross-domain ASTE is that the aspect terms, opinion terms, and sentiment polarities are of huge differences between the source and target domains. To tackle this problem, we propose  MultI-granularity ContrAstive learning (\methodwb) to align the fine-grained data distribution across domains. 
Since the aspect and opinion terms are phrases in a review and sentiments are the relations between the aspect and opinion terms, we employ contrastive learning to reduce the domain discrepancy from the perspective of phrases and aspect-opinion pairs.
Empirical results show that \method achieves the best performance, outperforming the state-of-the-art method by 4\% in the F1 score. \footnote{Our code will be available once accepted.}
\end{abstract}

==> chapters/1_introduction.tex <==
\section{Introduction}
Aspect Sentiment Triplet Extraction \citep[ASTE;][]{peng2020knowing} has become recently popular research. Prior works \citep{xu-etal-2021-learning, yan-etal-2021-unified} on ASTE heavily rely on supervised learning on massive labeled data. However, labeled data is hard to obtain since ASTE requires fine-grained annotation for each review. To alleviate the annotation cost, this paper studies the ASTE task in the cross-domain setting, which adapts models trained from a resource-rich source domain to a resource-poor target domain.

% The key challenge for cross-domain research is the domain discrepancy between the source and target domains. To alleviate this issue, previous approaches proposed in coarse-grained sentiment analysis and aspect-based sentiment analysis (ABSA) can be categorized into two frameworks:
% \XT{feature+ data based -> one /two }
% \begin{itemize}
%     \item \textbf{feature-based}. It focuses on learning domain-invariant feature that works well across domains \citep{blitzer-etal-2007-biographies, glorot2011domain, chernyshevich-2014-ihs, yu-jiang-2017-leveraging, ding2017recurrent, wang-pan-2018-recursive, ziser-reichart-2018-pivot, yang2019neural, wang-pan-2019-syntactically, ghosal-etal-2020-kingdom, gong-etal-2020-unified, zhang2021eatn}.
%     \item \textbf{data-based}. It aims to adjust the weight distribution of training data to better generalize to the target domain \citep{mansour2008domain, dredze2010multi, gong-etal-2020-unified}.
% \end{itemize}

The key challenge for cross-domain research is the domain discrepancy between the source and target domains \citep{blitzer2007biographies}. To alleviate this issue, previous approaches  propose to learn domain-invariant features \citep{yu-jiang-2017-leveraging, yang2019neural} or re-weight the source data to better generalize to the target domain \citep{li-etal-2012-cross}. 

However, these studies focus on sentence or aspect-level classification problems, which can not be directly adapted to the ASTE task. The domain discrepancy problem is more serious in the ASTE task because it contains three factors to be extracted and the triplets differ greatly across domains. For example, aspect terms in the restaurant domain mostly concern the \textit{food} or \textit{service} while those in the laptop domain are about \textit{power supply} or \textit{screen}. And opinion terms like \textit{delicious} or \textit{yummy} can rarely be seen in the laptop domain. Similarly, words like \textit{lightweight} and \textit{fast} in the laptop domain do not appear in the restaurant domain. 

% To address the challenge above, we propose a new domain adaptation strategy named MultI-level ContrAstive learning (\methodwb). \XT{describe this method with more details} Given reviews from different domains, we reduce the domain discrepancy from multiple levels. Specifically, for the phrases in each review, we enclose the distance of the aspect terms from different domains and the distance of the opinion terms from different domains. After obtaining the aspect-opinion pairs, we identify the sentiment polarity for each pair and employ contrastive learning to pull together the same sentiment.
% 正li
To address the challenge above, we propose a new domain adaptation strategy named MultI-granularity ContrAstive learning (\methodwb). Firstly, we employ contrastive learning (CL) \citep{jaiswal2020survey} to learn the domain-invariant features. CL is a common solution for representation learning. It learns semantics by encouraging the semantically similar positive pairs to be close to each other. Motivated by that, we construct positive pairs from the source and target domains. By pulling together the positive pairs, we can learn domain-invariant features. Secondly, since ASTE is a fine-grained task, triplets in ASTE are of huge differences across domains. We address the domain discrepancy in a multi-granularity way. Specifically, the aspect and opinion terms are phrases in a review, and sentiment polarities are the relations between the aspect and opinion terms. Therefore, we employ contrastive learning from the perspective of phrases and aspect-opinion pairs. In this way, we can align the source and target domains' aspect terms, opinion terms, and sentiments.


We evaluate \method on six transfer pairs of \citet{xu-etal-2020-position}. Results show that \method outperforms the  baseline model by 4\% in F1 scores. And quantitative analysis demonstrates that \method can reduce the domain discrepancy by 17\% and 10\%  for phrases and aspect-opinion terms, respectively.

==> chapters/2_related.tex <==
\section{Related Work}
\noindent\textbf{Cross-domain SA and Cross-domain ABSA.}
% Most of the previous works on cross-domain sentiment analysis (SA) and aspect-based sentiment analysis (ABSA) can be separated into two groups: feature-based and data-based methods. The \textbf{feature-based} methods focus on learning domain-invariant features that can generalize well across different domains. \citet{yu-jiang-2017-leveraging, yang2019neural, zhang2021eatn} leverage auxiliary tasks such as domain classification and sentiment detection to align the features from different domains. \citet{chernyshevich-2014-ihs, ziser-reichart-2018-pivot, wang-pan-2018-recursive, wang-pan-2019-syntactically} regard the part-of-speech and syntactic information as pivot feature that bridge the source and target domains. The \textbf{data-based} methods aim to re-weighting the training data, that is, assigning higher weights to the reviews or words similar to the target domain and lower weights to those different from the target domain. \citet{li-etal-2012-cross} construct pseudo-labeled data in the target domain, and re-weight the source data based on the pseudo-labeled data. \citet{gong-etal-2020-unified} combine the feature and data-based method. They first employ the part-of-speech features and syntactic relations to learn domain-invariant features, then perform word-level reweighting on the source data to better generalize to the target domain.
Most of the previous works on cross-domain sentiment analysis (SA) and aspect-based sentiment analysis (ABSA) can be separated into two groups: feature-based and data-based methods. The \textbf{feature-based} methods focus on learning domain-invariant features by leveraging auxiliary tasks like sentiment detection \citep{yu-jiang-2017-leveraging, yang2019neural, zhang2021eatn} and using pivot feature to bridge the source and target domains  \citet{chernyshevich-2014-ihs, ziser-reichart-2018-pivot, wang-pan-2018-recursive, wang-pan-2019-syntactically}. The \textbf{data-based} methods aim to re-weighting the training data, that is, assigning higher weights to the reviews or words similar to the target domain and lower weights to those different from the target domain. \citet{li-etal-2012-cross} construct pseudo-labeled data in the target domain, and re-weight the source data based on the pseudo-labeled data. \citet{gong-etal-2020-unified} propose a unified framework and combine the feature and data-based methods. 

However, these researches all focus on sentence or aspect-level classification problems, which can not be directly adapted to the ASTE task. ASTE concerns with more fine-grained sentimental information and the sentiment triplets between the source and target domain are of huge differences. Thus, we need a fine-grained domain adaptation strategy for cross-domain ASTE.

\paragraph{Contrastive Learning.} Contrastive learning has recently become a dominant solution  in self-supervised representation learning \citep{jaiswal2020survey}. It first constructs semantically similar positive pairs by data augmentation \citep{chen2020simple, misra2020self} and regards other instances in the dataset as negative examples. Then by pulling the positive pairs together and pushing the negative pairs away, it can learn semantics for the embedding. Motivated by studies in representation learning, we propose to apply contrastive learning to domain adaptation problems. By constructing positive and negative pairs from both the source and target domains, we can reduce the domain discrepancy.


==> chapters/3_method/backbone.tex <==
\subsection{Backbone Model}
Our backbone model is based on Span-ASTE \citep{xu-etal-2021-learning}, a representative model in ASTE. 
It first obtains the token representation through the encoding module, then extracts the aspect and opinion terms by predictions of the span module, and finally identifies the sentiment polarity in the pair module. 

\noindent\textbf{Encoding Module.} We use BERT \citep{devlin-etal-2019-bert} as the encoder to get contextualized token representations as follows:
\begin{equation}
    [\mathbf{h}_1, \mathbf{h}_2...,\mathbf{h}_n] = \mbox{BERT}(w_1, w_2,..., w_n)
    \label{eq:encode}
\end{equation}

\noindent\textbf{Span Module.} For all the phrases in the sentence, we define the span representation $\mathbf{s}_{i, j}$ by start token, end token, and width representations (Equation \ref{eq:span-rep}). Then we use the span-level representation to get scores for each span type $m\in \{Aspect, Opinion, Invalid\}$ (Equation \ref{eq:span-pred})
\begin{equation}
    \mathbf{s}_{i,j} = [\mathbf{h}_i; \mathbf{h}_j; f_{width}(i, j)]
    \label{eq:span-rep}
\end{equation}
\begin{equation}
    P(m|\mathbf{s}_{i, j})=\mbox{softmax}(\mbox{SPAN\_FFN}(\mathbf{s}_{i, j}))
    \label{eq:span-pred}
\end{equation}
where $f_{width}(i, j)$ produces a trainable feature embedding representing the span width. 
SPAN\_FFN denotes a feed-forward neural network with non-linear activation. 

Then we employ a pruning strategy to select candidates from the enumerated spans set $\text{SP}$ $(\forall \mathbf{s}_{i, j}\in \text{SP}, i < j)$ and obtain the aspect candidates $\widehat{\text{SP}}^a$ and the opinion candidates $\widehat{\text{SP}}^o$. Detailed pruning strategy can be seen in \citet{xu-etal-2021-learning}.

\noindent\textbf{Pair Module.} We obtain the aspect-opinion pair representation by performing Cartesian Product \citep{agesen1995cartesian} on $\widehat{\text{SP}}^a$ and $\widehat{\text{SP}}^o$ (Equation \ref{eq:pair-rep}). Then we obtain the sentiment relation $r\in \{Positive, Negative, Neutral, Invalid\}$ through a pair classifier (Equation \ref{eq:rel-pred}).
\begin{equation}
    \begin{split}
        % & \text{PAIR} = \widehat{\text{SP}}^a \otimes \widehat{\text{SP}}^o\\
        &\mathbf{g}_{\mathbf{s}_{b,c}^a, \mathbf{s}_{d,e}^o} = [\mathbf{s}_{b, c}^a; \mathbf{s}_{d,e}^o; f_{distance}(b, c, d, e)]
    \end{split}
    \label{eq:pair-rep}
\end{equation}
\begin{equation}
    P(r|\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o) = \text{softmax}(\text{PAIR\_FFN}(\mathbf{g}_{\mathbf{s}_{b,c}^a, \mathbf{s}_{d,e}^o}))
    \label{eq:rel-pred}
\end{equation}
where $\mathbf{s}_{b,c}^a\in \widehat{\text{SP}}^a, \mathbf{s}_{d,e}^o\in \widehat{\text{SP}}^o$, and $\mathbf{g}_{\mathbf{s}_{b,c}^a, \mathbf{s}_{d,e}^o}\in \text{PAIR}$, $\text{PAIR}$ is the set of all aspect-opinion pairs. $f_{distance}(b, c, d, e)$ produces a trainable feature embedding based on the distance  between the aspect and opinion spans. 
PAIR\_FFN is a feed-forward neural network with non-linear activation.

Finally, the training loss is defined as the sum of the negative log-likelihood from the span module and pair module.
\begin{equation}
    \begin{split}
        \mathcal{L}_{aste} = &- \sum_{\mathbf{s}_{i,j}\in \text{SP}^S} \log P(m=m_{i,j}^*|\mathbf{s}_{i,j}) \\
        &- \sum_{(\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o) \in \text{PAIR}^S}\log P(r=r^*|\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o)
    \end{split}
\end{equation}

% \begin{equation}
%     \begin{split}
%         \mathcal{L}_{aste} = &- \sum_{\mathbf{s}_{i,j}\in \text{SPAN}^S} \sum_k y(\mathbf{s}_{i, j})_k \log P(m|\mathbf{s}_{i,j})_k \\
%         &- \sum_{(\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o) \in \text{PAIR}^S}\log P(r^*|\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o)
%     \end{split}
% \end{equation}

where $r^*$ is the golden sentiment relation of the aspect and opinion span 
pair $(\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o)$, and $\text{SP}^S, \text{PAIR}^S$ only denote the span and pair sets from the source domain because the annotations are only available in the source domain.

==> chapters/3_method/backbone_v1.tex <==
\subsection{Backbone Model}
Our backbone model is Span-ASTE \citep{xu-etal-2021-learning}, a representative model in ASTE. 
It first obtains the token, span, and pair representations corresponding to the word, phrase, and aspect-opinion pair, respectively.
\begin{equation}
    \begin{split}
        [\mathbf{h}_1, \mathbf{h}_2...,\mathbf{h}_n] &= \mbox{BERT}(w_1, w_2,..., w_n)\\
        \mathbf{s}_{i,j} &= [\mathbf{h}_i; \mathbf{h}_j; f_{width}(i, j)]\\
        \mathbf{g}_{\mathbf{s}_{b,c}^a, \mathbf{s}_{d,e}^o} &= [\mathbf{s}_{b, c}^a; \mathbf{s}_{d,e}^o; f_{distance}(b, c, d, e)]\\
    \end{split}
    \label{eq:aste-rep}
\end{equation}
$\mathbf{s}_{i,j} \in \text{SP}$, $\text{SP}$ is the set of all candidate spans. Each span can be an aspect, opinion, or nothing. We conduct Cartesian Product \citep{agesen1995cartesian} on the candidate aspects and opinion to obtain pair representation $\mathbf{g}_{\mathbf{s}_{b,c}^a, \mathbf{s}_{d,e}^o}\in \text{PAIR}$, $\text{PAIR}$ is the set of all candidate aspect-opinion pairs.
$f_{width}(i, j)$ and $f_{distance}(b, c, d, e)$ are two embedding layers for the spans and pairs.


Then we employ the classifiers to get scores for each span type $m\in \{Aspect, Opinion, Invalid\}$ and pair type $r\in \{Positive, Negative, Neutral, Invalid\}$.
\begin{equation}
    \begin{split}
    &P(m|\mathbf{s}_{i, j})=\mbox{softmax}(\mbox{SPAN\_FFN}(\mathbf{s}_{i, j}))\\
    &P(r|\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o) = \text{softmax}(\text{PAIR\_FFN}(\mathbf{g}_{\mathbf{s}_{b,c}^a, \mathbf{s}_{d,e}^o}))
    \end{split}
    \label{eq:aste-prob}
\end{equation}

Finally, the training loss is defined as the sum of the negative log-likelihood from the span and pair representations.
\begin{equation}
    \begin{split}
        \mathcal{L}_{aste} = &- \sum_{\mathbf{s}_{i,j}\in \text{SP}^S} \log P(m=m_{i,j}^*|\mathbf{s}_{i,j}) \\
        &- \sum_{(\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o) \in \text{PAIR}^S}\log P(r=r^*|\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o)
    \end{split}
    \label{eq:aste-loss}
\end{equation}

where $r^*$ is the golden sentiment of the aspect-opinion pair $(\mathbf{s}_{b, c}^a, \mathbf{s}_{d, e}^o)$, and $\text{SP}^S, \text{PAIR}^S$ denote the span and pair sets from the source domain because the annotations are only available in the source domain.


==> chapters/3_method/contrastive.tex <==
\subsection{Fine-grained Contrastive Learning}

\noindent\textbf{Basic Intuition.} There are three key factors in the ASTE task, i.e., aspect terms, opinion terms, and sentiment polarity. They are of huge difference across domains. Therefore, we propose to alleviate the domain discrepancy through contrastive learning in a multi-granularity way. For the phrases in the review, we pull together the aspect terms from different domains and the opinion terms from different domains. For the aspect-opinion pair, we categorize them into different sentiments and pull together the pairs of the same sentiments.

\noindent\textbf{Positive and Negative Pairs.}  We draw the positive and negative pairs from both the source and target domains. Since there is no annotation for the target domain, we employ the pseudo label predicted by the backbone model, then pull features of the same type together and push features of different types away. Specifically, we employ an indicator function $c(\mathbf{x}_i, \mathbf{x}_j, t)$ for a feature $\mathbf{x}_i$ from the source domain and a feature $\mathbf{x}_j$ from the target domain. If $\mathbf{x}_j$ have the same prediction (with the prediction score higher than $t$) as $\mathbf{x}_i$, they are positive examples. Otherwise, they are negative examples.  

\noindent\textbf{Contrastive Learning.} Given the positive and negative features, we can obtain contrastive loss from the source-target and target-source directions:
\begin{equation}
\small
\begin{split}
    \mathcal{L}_{contra}(S, T, t) &= -\sum_{\mathbf{x}_i \in S} \sum_{\mathbf{x}_j\in T}\log\frac{d(\mathbf{x}_i, \mathbf{x}_j)c(\mathbf{x}_i, \mathbf{x}_j, t)}{\sum_{\mathbf{x}_k \in T}d(\mathbf{x}_i, \mathbf{x}_k)}\\
    &-\sum_{\mathbf{x}_i \in T} \sum_{\mathbf{x}_j\in S}\log\frac{d(\mathbf{x}_i, \mathbf{x}_j)c(\mathbf{x}_j, \mathbf{x}_i, t)}{\sum_{\mathbf{x}_k \in S}d(\mathbf{x}_i, \mathbf{x}_k)}\\\\
    d(\mathbf{x}_i, \mathbf{x}_j) &= \exp(\cos(\mathbf{x}_i, \mathbf{x}_j)/\tau)\\
\end{split}
\label{eq:contra-abs}
\end{equation}
where $\tau$ is the temperature hyperparameter, $S$ and $T$ are two feature sets from the source and target domains. 

Finally, we conduct contrastive learning on both span and pair-level representations. 
\begin{equation}
\small
    \begin{split}
        \mathcal{L}_{contra} &= \mathcal{L}_{contra}(SP^S, SP^T, t)\\
        &+\mathcal{L}_{contra}(PAIR^S, PAIR^T, t)
    \end{split}
    \label{eq:contar-all}
\end{equation}
The superscripts $S$ and $T$ denote the source and target domains, respectively.


==> chapters/3_method/formulation.tex <==
\subsection{Problem Formulation}
\noindent\textbf{ASTE.} Given an instance $\mathbf{x} = \{w_1, w_2,..., w_n\}$,  consisting of $n$ words, the goal of the ASTE task is to extract a set of sentiment triplets $\mathbf{y} = \{(a_1, o_1, s_1), ..., (a_i, o_i, s_i),...\}$ from the instance $\mathbf{x}$, where $a$, $o$ and $s$ denote the aspect term, opinion term, and sentiment polarity, respectively. 

==> chapters/3_method/main.tex <==
\section{Methodology}
\input{chapters/3_method/formulation.tex}
\input{chapters/3_method/backbone_v1.tex}
\input{chapters/3_method/contrastive.tex}
\input{chapters/3_method/objective.tex}

==> chapters/3_method/objective.tex <==
\subsection{Final Objective}
We merge the ASTE loss and contrastive loss in a joint way. The final training objective is:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{aste} + \lambda \mathcal{L}_{contra}
    \label{eq:final-loss}
\end{equation}
where $\lambda$ is the hyperparameter denoting the weight of contrastive loss.


==> chapters/4_experiment/analysis.tex <==
\subsection{Analysis}

\subsubsection{Ablation Study} \XT{wo pair/ wo phrase}
\XT{mv hyper-parameter to appendix}


\subsubsection{Quantitative Analysis}
To investigate the effectiveness of \method in reducing domain discrepancy, we perform quantitative analysis on the backbone model  and \methodwb. Specifically, we employ trained models to obtain the representation of phrases and aspect-pairs as shown in Equation \eqref{eq:aste-rep}. Then we compute the  Maximum Mean Discrepancy (MMD; \citealp{gretton2012kernel}) for both phrases and aspect-opinion pairs in Table \ref{tab:quantitative}. Finally, we observe that \method can reduce domain  discrepancy by 17\% and  10\% for phrases and aspect-opinion pairs, respectively, This implies that \method can learn better representations for cross-domain ASTE.

==> chapters/4_experiment/fig_ablation.tex <==
% \subsection{Challenges from ASTE}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/temperature.pdf}
     \end{subfigure}
        \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/threshold.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/weight.pdf}
     \end{subfigure}
        \caption{Ablation studies of sharpening temperature, pseudo-label threshold, and weight parameter.}
        \label{fig:hyper}
\end{figure*}


==> chapters/4_experiment/fig_quatitative.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/quatitative.pdf}
    \caption{Quantitative analysis for \methodwb. We demonstrate the domain discrepancy for both phrases and aspect-opinion pairs.}
    \label{fig:quatitative}
\end{figure}

==> chapters/4_experiment/main.tex <==
\section{Experiment}
\input{tables/main_result.tex}

% \input{chapters/4_experiment/fig_quatitative.tex}
\input{tables/quantitative.tex}
\input{chapters/4_experiment/setup.tex}
\input{chapters/4_experiment/main_result.tex}
\input{chapters/4_experiment/analysis.tex}

==> chapters/4_experiment/main_result.tex <==
\subsection{Main Results}
 We report the F1 scores of various methods on six transfer pairs of \citet{xu-etal-2021-learning} in Table \ref{tab:main-result}. From the table we make the following observations: (1)Comparing Span-ASTE with all other baseline models, we can see that Span-ASTE generally performs the best. This is the reason we design domain adaptation mechanisms based on Span-ASTE. (2) Compared with Span-ASTE, \method is 4\% higher in terms of the average performance of all transfer pairs. And it achieves consistent improvement over most of the transfer pairs. 
(3) Compared with the adversarial training, \method achieves significantly better performance  of all transfer pairs. It indicates that \method can learn better features for domain adaptation.
% (4) Of all the target domains, \method obtains the most performance gains when transferring to the Book domain. We think the reason is that the Book domain is very different from other source domains.  

==> chapters/4_experiment/setup.tex <==
\subsection{Experimental Setup}
\noindent\textbf{Datasets.} We evaluate \method on the ASTE dataset from \citet{xu-etal-2021-learning}. It contains data from two domains, i.e., restaurant and laptop. We construct six transfer pairs based on the dataset and conduct cross-domain experiments on them.

\noindent\textbf{Baselines.} We compare \method with several highly competitive ASTE methods. (1) BMRC \citep{chen2021bidirectional}: a machine reading comprehension (MRC) method with bidirectional query. (2) BART-ABSA \citep{yan-etal-2021-unified}: a generative-based method with pointer network. (3) GTS \citep{wu-etal-2020-grid}: a grid tagging method that encode the review into a 2D grid and decode the triplet information from the grid. (4) Span-ASTE \citep{xu-etal-2021-learning}: a tagging-based method that first extracts the aspect and opinion terms and then identifies the sentiment. Moreover, we incorporate some of these methods with domain adversarial training (AT), a dominant solution in domain adaptation scenarios. (1) BMRC + AT: BMRC with adversarial training at the token level. (2) Span-ASTE + AT: Span-ASTE with adversarial training in the token level.

\noindent\textbf{Implementation Details.} We train the model with labeled data from the source domain and unlabeled data from the target domain.   We use AdamW optimizer \citep{loshchilov2017decoupled}. The learning rates for BERT and classifier are set to $5\cdot 10^{-5}$ and $1\cdot 10^{-3}$, respectively. We perform grid-research for the hyper-parameters. All these hyperparameters are tuned on the validation set.

\noindent\textbf{Evaluation Metric.} In our study, we employ F1 score to measure the performance of different approaches. Following prior works \citep{xu-etal-2021-learning}, only extract match can be considered correct.  All experiments are repeated five times with random seeds from 0 to 4. 

==> chapters/5_conclusion.tex <==
\section{Conclusion}
We propose \methodwb, a novel method for cross-domain ASTE. The method focuses on reducing the domain discrepancy between the source and target domains in a multi-granularity way. Specifically, we employ contrastive learning to learn domain-invariant features for both phrases and aspect-opinion pairs. Empirical experiments show that \method outperforms the state-of-the-art model by 4\% in the F1 score. 

==> chapters/6_limitation.tex <==
\section*{Limitations}
The limitation of this study is the limited evaluation scenarios. In the experiments, we evaluate the performance when transferring from the restaurant domain to the laptop domain and from the laptop domain to the restaurant domain since restaurant and laptop are the only two domains available in existing datasets. Future works can validate the model performances on more diversified transfer pairs. 

==> chapters/main.tex <==
\newcommand\XT[1]{\textcolor{red}{\{XT: #1 \}}}
\newcommand{\method}{\textsc{MICA }}
\newcommand{\methodwb}{\textsc{MICA}}
\input{chapters/0_abstract.tex}
\input{chapters/1_introduction.tex}
\input{chapters/2_related.tex}
\input{chapters/3_method/main.tex}
\input{chapters/4_experiment/main}
\input{chapters/5_conclusion.tex}
\input{chapters/6_limitation.tex}

\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\input{chapters/6_appendix/main.tex}


==> chapters_0110/0_abstract.tex <==
\begin{abstract}
% cross-domain aste is important but not well explored
Aspect Sentiment Triplet Extraction (ASTE) has achieved promising results while relying on sufficient annotation data in the specific domain. 
Meanwhile, ASTE is a fine-grained understanding task, covering aspect, opinion, and sentiment polarity triplet, which makes it challenging to handle the domain discrepancy. Therefore, we propose the Fine-grained cOntrAstive Learning (\methodwb) method to reduce the domain discrepancy by constructing cross-domain positive and negative pairs at the phrase and pair level.
\method constructs cross-domain positive and negative pairs based on the type of phrase and phrase pair.
Experiments on six transfer pairs show \method outperforms the baseline model by 4\% in F1 scores and reduces the domain discrepancy significantly.
\end{abstract}

==> chapters_0110/1_introduction.tex <==
\section{Introduction}
Aspect Sentiment Triplet Extraction \citep[ASTE;][]{peng2020knowing}, a fine-grained sentiment analysis \XT{citation} task, has attracted considerable interest recently. It focuses on extracting the sentiment triplets from a given review, ie., aspect terms, opinion terms, and sentiment polarity. Prior works \citep{xu-etal-2021-learning, yan-etal-2021-unified} on ASTE have achieved promising results while heavily rely on sufficient annotation data in the specific domain.
% and can generalize well to new data which is drawn from the same distribution as the training data. 

% However, in many cases, we may have a massive amount of labeled data for a \textit{source} domain, but we need to process reviews from a \textit{target} domain, which shares different data distribution from the \textit{source} domain and has no annotations \XT{citation}. Therefore, we propose to investigate ASTE in the cross-domain setting, which adapts a model trained on a resource-rich source domain for use in a resource-poor target domain.

% 然而，在现实场景中，将ASTE应用到开放环境中是必要的。开放环境下，
% However, the ASTE model is always applied to an open environment \XT{modify, citation}, which processes reviews drawn from a domain with a distribution different from the training data. Therefore, we propose to investigate ASTE in the cross-domain setting\XT{citation}, which adapts a model trained on a resource-rich \textit{source} domain for use in a resource-poor \textit{target} domain.

However, in reality, reviews often come from diverse domains (e.g. Amazon Review \citep{ni-etal-2019-justifying} covers 29 domains). It is unrealistic to annotate an adequate amount of data for each domain. Cross-domain transfer learning \citep{pan2009survey} provides an effective way to transfer knowledege from resource-rich \textit{source} domain to a resource-poor \textit{target} domain, which alleviates the dependence on labeled data in the target domain. Therefore, it's crucial to explore the domain adaptation method on ASTE task. 

%\XT{细粒度准确的迁移能力}
% The key challenge for cross-domain ASTE is the fine-grained domain discrepancy across domains. \XT{specifically,} Because source data and target data are drawn from different distributions,  domain discrepancy exists between the two domains. For cross-domain ASTE, domain discrepancy comes from the aspect terms, opinion terms, and sentiment polarities because \XT{because?} they are three key factors for ASTE.  For example, aspect terms in the restaurant domain mostly concern the \textit{food} or \textit{service} while those in the laptop domain are about \textit{power supply} or \textit{screen}. And opinion terms like \textit{delicious} or \textit{yummy} can rarely be seen in the laptop domain. Similarly, words like \textit{lightweight} and \textit{fast} in the laptop domain do not appear in the restaurant domain. To summarize, we need to answer a question to address cross-domain ASTE: \textit{(1) How to reduce the domain discrepancy from the perspective of the aspect terms, opinion terms, and sentiment polarities?}

The key challenge for cross-domain ASTE is the fine-grained discrepancy across domains. 
Reducing the representation discrepancy between domains is an effective and straightforward way to improve the cross-domain transfer performance\citep{ganin2016domain}.
Many such domain adaptation approaches\citep{} align the overall representation distribution of the source domain and target domain without considering the discrepancy within the sequence. 
In cross-domain ASTE task, the domain discrepancy comes from three factors: the aspect terms, opinion terms, and sentiment polarities.  For example, aspect terms in the restaurant domain mostly concern the \textit{food} or \textit{service} while those in the laptop domain are about \textit{power supply} or \textit{screen}. And opinion terms like \textit{delicious} or \textit{yummy} can rarely be seen in the laptop domain. Similarly, words like \textit{lightweight} and \textit{fast} in the laptop domain do not appear in the restaurant domain.
Therefore, it is challenging to reduce the domain discrepancy in the ASTE task.

% To answer the question, we propose a new domain adaptation strategy named Fine-grained cOntrAstive Learning (\methodwb), \textit{contrastive learning} to reduce domain discrepancy and \textit{fine-grained} to align the three factors across domains. Specifically, contrastive learning \XT{citation} has been applied to the domain adaptation scenarios recently \XT{citation}. However, these studies focus on coarse-grained tasks like image classification \XT{citation} and sentiment classification\XT{citation}, which is not adequate to reduce a fine-grained domain discrepancy\XT{why}. Therefore, we propose to utilize contrastive learning in a fine-grained way. 
% \XT{why?} To be specific, we first regard the aspect and opinion terms as phrases in a review and regard sentiment polarities as relations of the aspect-opinion pairs. Then we employ contrastive learning from the perspectives of phrases and aspect-opinion pairs. \XT{advantages}
% 好处有什么

To address aforementioned challenge in cross-domain ASTE task, we propose the Fine-grained cOntrAstive Learning (\methodwb), which handlers the domain discrepancy in multiple granularity.
Contrastive learning\citep{chen2020simple} aligns the representation of the positive pair to be close to each other while making the negative pair apart.
It provides a flexible way to reduce the representation discrepancy at specific levels by constructing corresponding positive and negative instances.
In cross-domain ASTE task, we construct the positive pair for spans with the same type (aspect, opinion or invalid) and negative pair with different types.
For the sentiment polarity, we construct the positive pair for aspect-opinion pair with the same polarity class (positve, negative, neutral or invalid) and negative pairs with different classes.
All positive and negative pairs are across different domains.
By constructing positive and negative pairs at multiple granularity, \method can reduce the fine-grained domain discrepancy. 

% To address the challenge above, we propose a new domain adaptation strategy named MultI-granularity ContrAstive learning (\methodwb). Firstly, we employ contrastive learning (CL) \citep{jaiswal2020survey} to learn the domain-invariant features. CL is a common solution for representation learning. It learns semantics by encouraging the semantically similar positive pairs to be close to each other. Motivated by that, we construct positive pairs from the source and target domains. By pulling together the positive pairs, we can learn domain-invariant features. Secondly, since ASTE is a fine-grained task, triplets in ASTE are of huge differences across domains. We address the domain discrepancy in a multi-granularity way. Specifically, the aspect and opinion terms are phrases in a review, and sentiment polarities are the relations between the aspect and opinion terms. Therefore, we employ contrastive learning from the perspective of phrases and aspect-opinion pairs. In this way, we can align the source and target domains' aspect terms, opinion terms, and sentiments.


We evaluate \method on six transfer pairs of \citet{xu-etal-2020-position}. Results show that \method outperforms the baseline model by 4\% in F1 scores. And quantitative analysis demonstrates that \method can reduce the domain discrepancy by 17\% and 10\%  for phrases and aspect-opinion terms, respectively.

==> chapters_0110/2_related.tex <==
\section{Related Work}

% ASTE

% Crosss-domain Transfer Learning

==> chapters_0110/main.tex <==
\newcommand\XT[1]{\textcolor{red}{\{XT: #1 \}}}
\newcommand{\method}{\textsc{FOAL }}
\newcommand{\methodwb}{\textsc{FOAL}}
\input{chapters_0110/0_abstract.tex}
\input{chapters_0110/1_introduction.tex}
\input{chapters/3_method/main.tex}
\input{chapters/4_experiment/main}
\input{chapters_0110/2_related.tex}
\input{chapters/5_conclusion.tex}
\input{chapters/6_limitation.tex}

\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\input{chapters/6_appendix/main.tex}

==> chapters_0115/2_related.tex <==
a

==> chapters_0115/3_method/formulation.tex <==
\subsection{Task Definition}
\noindent\textbf{ASTE.} Given an instance $\mathbf{x} = \{w_1, w_2,..., w_n\}$,  consisting of $n$ words, the goal of the ASTE task is to extract a set of sentiment triplets $\mathbf{y} = \{(a_1, o_1, s_1), ..., (a_i, o_i, s_i),...\}$ from the instance $\mathbf{x}$, where $a$, $o$ and $s$ denote the aspect term, opinion term, and sentiment polarity, respectively. 

==> tables/ablation_quantitative.tex <==
\begin{table*}[]
    \centering
    \small
    \begin{tabular}{lcccc}
    \toprule
         Method & Span-ASTE & \method & \method only phrase-level & \method only pair-level  \\
    \midrule
         & \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
